Sandra -- A Neuro-Symbolic Reasoner Based On Descriptions And Situations

This paper presents sandra, a neuro-symbolic reasoner combining vectorial representations with deductive reasoning. Sandra builds a vector space constrained by an ontology and performs reasoning over it. The geometric nature of the reasoner allows its combination with neural networks, bridging the gap with symbolic knowledge representations. Sandra is based on the Description and Situation (DnS) ontology design pattern, a formalization of frame semantics. Given a set of facts (a situation) it allows to infer all possible perspectives (descriptions) that can provide a plausible interpretation for it, even in presence of incomplete information. We prove that our method is correct with respect to the DnS model. We experiment with two different tasks and their standard benchmarks, demonstrating that, without increasing complexity, sandra (i) outperforms all the baselines (ii) provides interpretability in the classification process, and (iii) allows control over the vector space, which is designed a priori.

==> sections/experiments_reasoner.tex <==

We consider three types of situations: commercial transaction ($CT$), refund ($R$), and commerce buy ($CB$). 
In particular $R$ and $CB$ specialises $CT$, namely, they require the same set of necessary roles from $CT$, with the addition of at least one specific necessary role for each $CB$ and $R$.
Considering the formalisation mentioned in Section \ref{sec:method}, being $R$ and $CB$ Descriptions, and $ct$ a Situation fully satisfying the $CT$ description, $R$ and $CB$ are \emph{quasi-satisfied} by a $ct$ situation, which, being more general, namely, requiring fewer or less specified components (roles).

The conversion of situations that are designed to satisfy $R$ and $CB$ into points in the vector space $V$ is exemplified. If a situation can be expressed as linear combination of a description’s components (α, β, γ ̸ = 0) then it satisfies that description.

For the purpose of testing \emph{sandra} we model in OWL2 the above mentioned example introducing $R$, $CB$ and $CT$ as classes of situation, specifically \texttt{:Refund} and \texttt{:CommerceBuy} are declared as \texttt{rdfs:subClassOf} \texttt{:CommercialTransaction}.



\begin{itemize}
    \item Introduce ontology toy example of DnS
    There is a set of situations interpretable from several perspectival interpretations, 
    
    \item it is subset of PropBank frames
    \item Show Commerce\_buy, Importer etc example
    \item Make nice figure that exemplifies of the reasoner works in a graphical way and also shows the results
    \item implementation is freely available on github and the example is there - every one can play with it
\end{itemize}
